On-Device LLM for Context-Aware Wi-Fi Roaming

Roaming in Wireless LAN (Wi-Fi) is a critical yet challenging task for maintaining seamless connectivity in dynamic mobile environments. Conventional threshold-based or heuristic schemes often fail, leading to either sticky or excessive handovers. We introduce the first cross-layer use of an on-device large language model (LLM): high-level reasoning in the application layer that issues real-time actions executed in the PHY/MAC stack. The LLM addresses two tasks: (i) context-aware AP selection, where structured prompts fuse environmental cues (e.g., location, time) to choose the best BSSID; and (ii) dynamic threshold adjustment, where the model adaptively decides when to roam. To satisfy the tight latency and resource budgets of edge hardware, we apply a suite of optimizations-chain-of-thought prompting, parameter-efficient fine-tuning, and quantization. Experiments on indoor and outdoor datasets show that our approach surpasses legacy heuristics and DRL baselines, achieving a strong balance between roaming stability and signal quality. These findings underscore the promise of application-layer LLM reasoning for lower-layer wireless control in future edge systems.

==> section/conclusion.tex <==
\section{conclusion} \label{sec:conclusion}





==> table/ablation_task1.tex <==
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\begin{tabular}{l|ccc|ccc}
\toprule[1.5pt]
\textbf{Combination} & \textit{\textbf{Loc}} & \textit{\textbf{TS}} & \textit{\textbf{BC}} & \textbf{\# Handover} & \textbf{Avg. RSSI (dBm)} & \textbf{Error Rate (\%)} \\
\midrule[.8pt]
w/o Context & \xmark & \xmark & \xmark & 102 & -59.93 & 26.19 \\
\cmidrule(lr){1-7}
TS + BC & \xmark & \cmark & \cmark & 99 & -59.73 & 24.43 \\
Loc + BC & \cmark & \xmark & \cmark & 101 & -58.97 & 26.82 \\
Loc + TS & \cmark & \cmark &  \xmark & 98 & -59.17 & 19.68 \\
\cmidrule(lr){1-7} 
\texttt{w/ All} & \cmark & \cmark & \cmark & 94 & -60.11 & 22.32 \\
\bottomrule[1.5pt]
\end{tabular}

==> table/parameter_DPO.tex <==
  \begin{tabular} {l l | l l}
	\toprule[1pt]
	\textbf{Parameter} & \textbf{Value} & \textbf{Parameter} & \textbf{Value} \\
	% \cmidrule(lr){1-1} \cmidrule(lr){2-2}
        \midrule
        % Base model & Meta Llama 3 8B Instruct\\
	Learning rate & 5e-5 & Weight decay & 0.01\\  
	Batch size & 1 & Dropout & 0\\  
        Gradient accumulation steps & 4 & Max sequence length & 3000\\
        Beta & 0.2 & \# of epochs & 1\\
	LoRA rank & 16 & Optimizer & AdamW\\
        LoRA alpha & 16 & &\\
	\bottomrule[1pt]
  \end{tabular}
